High Throughput Push Based Storage Manager

The storage manager, as a key component of the database system, is responsible for organizing, reading, and delivering data to the execution engine for processing. According to the data serving mechanism, existing storage managers are either pull-based, incurring high latency, or push-based, leading to a high number of I/O requests when the CPU is busy. To improve these shortcomings, this thesis proposes a push-based prefetching strategy in a column-wise storage manager. The proposed strategy implements an efficient cache layer to store shared data among queries to reduce the number of I/O requests. The capacity of the cache is maintained by a time access-aware eviction mechanism. Our strategy enables the storage manager to coordinate multiple queries by merging their requests and dynamically generate an optimal read order that maximizes the overall I/O throughput. We evaluated our storage manager both over a disk-based redundant array of independent disks (RAID) and an NVM Express (NVMe) solid-state drive (SSD). With the high read performance of the SSD, we successfully minimized the total read time and number of I/O accesses.

==> accessModel.tex <==
%\subsection{Data Chunk}\label{dataChunk}
%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[htbp]
%	\centering
%	\includegraphics[width=0.65\textwidth]{./figures/FileVer}
%	\caption{Horizontal partition.}
%	\label{fig:filePartition}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%
%% The definition of the data chunk, describe our own structure the chunk, veritcal + horizontal 
%Chunking refers to a storage layout which combines the merits of row-store and column store together. Chunking divides data into equivalent, elementary chunks of data\ref{fig:filePartition}, which is horizontal data partitioning strategy of data parallelism. When executing a query, the partitions are independently assigned to different execution entities for processing. Since each processing entity works on a considerably smaller dataset, a speed-up proportional to the number of processing workers can be obtained in optimal conditions. Data partitioning can be applied both to the raw files as well as to the internal processing representation. We apply the simple data partitioning strategy described in~\cite{dewitt-paralleldb} by breaking the raw file into multiple segments of fixed size---in the order of tens to hundreds of megabytes. This has the potential to increase the length of sequential scans and reduce the number of disk seeks. The segment, i.e., chunk, is both the read/write and processing unit.
%
%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[htbp]
%	\centering
%	\includegraphics[width=0.65\textwidth]{./figures/ChunkOnly}
%	\caption{Chunk structure for internal processing.}
%	\label{fig:chunk-structure}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%
%
%Figure~\ref{fig:chunk-structure} depicts the generic structure of an internal chunk we apply column-based storage inside chunks. This type of storage structure vertically partitions columns inside chunks, associated with an array of pointers to all the columns. The actual data are vertically partitioned, with each column stored in a separate set of disk blocks. This design can improve the performance for accessing selective attributes and allows only for the required columns to be read for each query, thus minimizing the I/O bandwidth. Chunks also serve as the basic unit of parallelism, since different chunks can be sent to different CPU cores for processing.
%
%The chunk size play important role in data partition process, which could heavily impact the system performance. Small chunks lead to a more even distribution of data at the expense of more frequent migrations. This incurs high cost for data routing. Large chunks lead to fewer migrations. This is more efficient both from the networking perspective and in terms of internal overhead at the query routing layer. But, these efficiencies come at the expense of a potentially uneven distribution of data.  
%
%Given a huge data set, the data would be firstly divided into multiple data chunks. Assume the total number of tuples is $N$ and the size of data chunk is $n$, then the number of chunks would be $ceil(N/n)$, with chunk id from $0\ to\ ceil(N/n) - 1$. The number of columns is decided by the number of attribution in the data. In this layout, the combination of chunk id and column id can be used to define the basic unit of the data in our system, which is a single column inside a chunk. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Parallel Computation}\label{sec:parallelism}
%Parallel computing is a form of computation in which many calculations are carried out simultaneously, operating on the principle that large problems can often be divided into smaller ones, which are then solved concurrently. In this section, we present how to utilize parallelism to speed-up in-situ data processing. We recognize three general types of parallelization~\cite{dewitt-paralleldb}: data parallelism, task parallelism, and pipelining. In the following sections, we introduce these parallelization methods and show how they apply to storage manager. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\paragraph*{Data partitioning}
%Horizontal data partitioning or chunking is one strategy of data parallelism. When executing a query, the partitions are independently assigned to different execution entities for processing. Since each processing entity works on a considerably smaller dataset, a speed-up proportional to the number of processing workers can be obtained in optimal conditions. Data partitioning can be applied both to the raw files as well as to the internal processing representation. We apply the simple data partitioning strategy described in~\cite{dewitt-paralleldb} by breaking the raw file into multiple segments of fixed size---in the order of tens to hundreds of megabytes. This has the potential to increase the length of sequential scans and reduce the number of disk seeks. The segment, i.e., chunk, is both the read/write and processing unit.

%Figure~\ref{fig:chunk-structure} depicts the generic structure of an internal  chunk containing metadata to support range-based data partitioning. The metadata contains the minimum and maximum values for each attribute and are stored in the system catalog. They represent a primitive form of indexing. Besides, we further apply column-based storage inside chunks. This type of storage structure vertically partitions columns inside chunks, associated with an array of pointers to all the columns. The actual data are vertically partitioned, with each column stored in a separate set of disk blocks. This design can improve the performance for accessing selective attributes and allows only for the required columns to be read for each query, thus minimizing the I/O bandwidth. However, the impact of the (Min, Max) ranges on attributes is not always significant since there is no guarantee that attribute values are clustered. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Task Parallelism}\label{sec:parallelism:task}
%Task parallelism\footnote{\url{http://en.wikipedia.org/wiki/Task\_parallelism}} -- also known as function parallelism or control parallelism -- is a form of parallelization of computer code across multiple processors in parallel computing environments. Task parallelism focuses on distributing execution processes -- or threads -- across different parallel computing nodes. Task parallelism can be applied to raw file query processing by assigning the stages identified in Figure~\ref{fig:storage-arch} -- \texttt{TableScanner}, \texttt{ChunkReader}, \texttt{DiskArray} and \texttt{HD Thread} -- to separate processes or threads. In modern multi-core CPUs, different stages -- and multiple instances of the same stage -- can be executed concurrently. Moreover, query processing can be viewed as another task that can be also included in the parallel task assignment process.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Pipelining}\label{sec:parallelism:pipeline}
%Pipeline parallelism is a special form of task parallelism where a problem is divided into sub-problems, which can each be operated on independently, and where there are multiple problem instances to be solved at a given instant in time. Compared to data parallelism, this approach causes shorter latency, less buffering, and good locality. The potential benefits of pipeline parallelism are easy to quantify. Assuming an application is divided into $n$ stages, let $t_i$ denote the processing time for each stage. Then, the execution time and throughput for a non-pipelined program are $T_{\textit{no-pipeline}} = \sum_{i=1}^{n} t_i$ and $1/T_{\textit{no-pipeline}}$, respectively. When pipeline parallelism is active, suppose $t_m = \max \{t_1, t_2, \dots, t_n\}$ represents the execution time of the slowest stage in the pipeline. Then, the pipeline throughput is $1/t_m$, since a result is produced at every $T_{\textit{pipeline}} = t_m$ time instances. When executing a set of $L$ tasks, the speedup rate is given by:
%\begin{equation}\label{fun:speedup}
%\begin{aligned}
%\eta = \frac{L\cdot T_{\textit{no-pipeline}}} {T_{\textit{no-pipeline}} + (L-1) \cdot t_m}
%\end{aligned}
%\end{equation}
%When the number of tasks L is extremely large, i.e., $L \rightarrow \infty$, the speedup approaches $T_{\textit{no-pipeline}}/t_m$, which means the pipeline throughput is decided entirely by the slowest stage.
%
%Pipeline parallelism can be exploited by mapping clusters of producers and consumers to different stages, connected through buffers. Buffering allows storing results of a stage temporarily before forwarding them to the subsequent stages. It is essential in smoothing out the flow of a computational process when the timing for each stage is variable.






==> rel-work.tex <==
\section{Related Work}\label{sec:rel-work}

Several researchers~\cite{gray:scientific-data,ailamaki:scientific-data,stonebraker:science-data,kersten:data-deluge} have recently identified the need to reduce the analysis time for processing tasks operating over massive repositories of raw data. In-situ processing~\cite{grep-vs-flat-vs-mysql} has been confirmed as one promising approach. At a high level, we can group in-situ data processing into two categories. In the first category, we have extensions to traditional database systems that allow raw file processing inside the execution engine. Examples include external tables~\cite{oracle:external-tables,datastage} and various optimizations that eliminate the requirement for scanning the entire file to answer the query~\cite{files-queries-results,nodb,data-vaults}. The second category is organized around the MapReduce programming paradigm~\cite{google:mapreduce} and its implementation in Hadoop. While some of the data extraction is implemented by adapters that convert data from various representations into the Hadoop internal format\footnote{\url{https://github.com/julianhyde/optiq}}, the application is still responsible for a significant part of the conversion, i.e., the Map and Reduce functions contain large amounts of tokenizing and parsing code. The work in this category focuses on eliminating the conversion code by caching the already converted data in memory or storing it in binary format inside a database~\cite{invisible-loading}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\paragraph*{\texttt{SCANRAW}~\cite{scanraw}}
%The \texttt{SCANRAW} meta-operator is introduced in~\cite{scanraw}. The super-scalar pipeline architecture is designed following a detailed analysis of the conversion process from the raw file representation to the processing format. Speculative loading is proposed as an adaptive mechanism to load data into the database whenever there is spare disk I/O throughput---and without interfering with query processing. In this work, we bring three novel contributions that enhance the functionality of the \texttt{SCANRAW} meta-operator significantly and provide a deeper understanding of how to process raw files efficiently on modern computer architectures. First, in addition to data partitioning parallelism and pipelining, we also integrate vectorized SIMD instructions, as a new form of parallelism supported by the instruction sets of modern CPUs, in \texttt{SCANRAW}. After carefully considering all the stages of the extraction process, we identify \texttt{TOKENIZE} as the only stage where vectorization provides a significant performance boost. Second, we design two scheduling strategies for assigning worker threads to tasks. Best-effort scheduling satisfies the requests in the order in which they are received by the scheduler---without considering additional data. Adaptive scheduling takes into consideration the state of the entire system when assigning worker threads. The goal is to optimize resource utilization in the system and minimize query execution time, while maximizing the amount of data loaded into the database. And finally, we consider alternative strategies for processing queries when the same data are stored both in the raw file, as well as inside the database. We design the merge read strategy which combines reading data from two sources optimally by grouping multiple requests corresponding to the same source and scheduling them together. In addition to formalizing the concepts introduced by each of the proposed contributions, we also present extensive experimental results that quantify their relevance across the overall \texttt{SCANRAW} architecture.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph*{External tables}
Modern database engines, e.g., Oracle and MySQL, provide external tables as a feature to directly query flat files using SQL without paying the upfront cost of loading the data into the system. External tables work by linking a database table with a specified schema to a flat file. Whenever a tuple is required during query processing, it is read from the flat file, parsed into the internal database representation, and passed to the execution engine. Our work can be viewed as a parallel pipelined implementation of external tables that takes advantage of the current multi-core processors for improving performance significantly when mapping data into the processing representation is expensive. As far as we know, \texttt{SCANRAW} is the first parallel pipelined solution for external tables in the literature. Moreover, \texttt{SCANRAW} goes well beyond the external tables functionality and supports speculative loading, tokenizing, and parsing.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph*{Adaptive partial loading~\cite{files-queries-results}}
The main idea in adaptive partial loading is to avoid the upfront cost of loading the entire data into the database. Instead, data are loaded only at query time and only the attributes required by the query, i.e., push-down projection. An additional optimization aimed at further reducing the amount of loaded data is to push the selection predicates into the loading operator, i.e., push-down selection, such that only the tuples participating in the other query operators are loaded. The proposed adaptive loading operator is invoked whenever columns or tuples required in the current query are not stored yet in the database. It is important to notice that the operator executes a partial data loading before query execution can proceed. While \texttt{SCANRAW} supports adaptive partial loading, it avoids loading all the data into the database the first time they are accessed. Query processing has higher priority. Data are loaded only if sufficient I/O bandwidth is available.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph*{NoDB~\cite{nodb}}
NoDB never loads data into the database. It always reads data from the raw file thus incurring the inherent overhead associated with tokenizing and parsing. Efficiency is achieved by a series of techniques that address these sources of overhead. Caching is used extensively to store data converted in the database representation in memory. If all data fit in memory NoDB operates as an in-memory database, without accessing the disk. Whenever data have to be read from the raw file, tokenizing and parsing have to be executed. This is done adaptively though. A positional map with the starting position of all the attributes in all the tuples completely eliminates tokenizing. The positional map is built incrementally, from the executed queries. Moreover, only the attributes required in the current query are parsed. When the positional map, selective parsing, and caching are put together, NoDB achieves performance comparable -- if not better -- to executing queries over data stored in the database. This happens though only when NoDB operates over cached data, as an in-memory database. The main difference between \texttt{SCANRAW} and NoDB is that \texttt{SCANRAW} still loads data into the databases---without paying any cost for it though. Additionally, \texttt{SCANRAW} implements a parallel pipeline for data conversion. This is not the case in NoDB which is implemented as a PostgreSQL extension.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph*{Data vaults~\cite{data-vaults}}
Data vaults apply the same idea of query-driven just-in-time caching of raw data in memory. They are used in conjunction with scientific repositories though and the cache stores multi-dimensional arrays extracted from various scientific file formats. Similar to NoDB, the cached arrays are never written to the database. The ability to execute queries over relations stored in the database, cached arrays, and scientific file repositories using SciQL as a common query language is the main contribution brought by data vaults.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph*{Invisible loading~\cite{invisible-loading}}
Invisible loading extends adaptive partial loading and caching to MapReduce applications which operate natively over raw files stored in a distributed file system. The database is used as a disk-based cache that stores the content of the raw file in binary format. This eliminates the inherent cost of tokenizing and parsing data for every query. Notice though that processing is still executed by the MapReduce framework, not the database. Thus, the database acts only as a more efficient storage layer. In invisible loading, data converted into the MapReduce internal representation are first stored in the database and only then are passed for processing. While this is similar to adaptive partial loading~\cite{files-queries-results}, an additional optimization is aimed at reducing the storing time. Instead of saving all the data into the database, only a pre-determined fraction of a file is stored for every query. The intuition is to spread the cost of loading across multiple queries and to make sure that loaded data are indeed used by more than a single query. The result is a smooth decrease in query time instead of a steep drop after the first query---responsible for loading all the required data. The proposed speculative loading implemented in \texttt{SCANRAW} brings two novel contributions with respect to invisible loading. First, the amount of data loaded for every query changes dynamically based on the available system resources. Speculative loading degenerates to invisible loading only in the case when no I/O bandwidth is available. And second, speculative loading overlaps entirely with query processing without having any negative effects on query performance. This is the result of the \texttt{SCANRAW} pipelined architecture.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph*{Instant loading~\cite{instant-loading}}
Instant loading proposes scalable bulk loading methods that take full advantage of the modern super-scalar multi-core CPUs. Specifically, vectorized implementations using \texttt{SSE 4.2} SIMD instructions are proposed for tokenizing. The extraction stages are still executed sequentially though, for every data partition---there is no pipeline parallelism. Moreover, instant loading does not support query processing over raw files. \texttt{SCANRAW}, on the other hand, overlaps the execution of tokenizing and parsing both across data partitions, and for each partition individually. And with the actual query processing and/or loading. Overall, instant loading introduces faster algorithms for tokenizing that we integrate in \texttt{SCANRAW}. While the benefits of vectorization are evident when \texttt{TOKENIZE} is considered in isolation, the impact on the overall query execution is limited to the percentage tokenization represents from the total. As our detailed stage analysis shows, tokenization represents only a small fraction since parsing dominates the extraction time. Consequently, the impact vectorization has on in-situ raw file data processing is considerable only in specific scenarios, e.g., the file consists of a large number of text attributes that do not require parsing.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph*{SDS/Q~\cite{blanas:sigmod-2014}}
SDS/Q executes queries directly over data stored in HDF5 files. Similar to NoDB, it never loads data into the database. Instead, it always reads data from the raw file. However, since HDF5 is a binary storage format, in most cases, the parse and tokenize stages can be omitted. Moreover, SDS/Q builds external bitmap indexes to eliminate the requirement for scanning the entire file in order to reduce query response time. Compared to SDS/Q, \texttt{SCANRAW} can not only process queries directly from scientific raw files in binary format -- HDF5 is only one such example -- but can also execute queries from other file formats, including text files. Furthermore, due to the parallel pipeline for data conversion, \texttt{SCANRAW} can load data into the databases whenever necessary---and without paying any cost for it. This is not supported in SDS/Q, which is a distributed shared-memory data processing system without secondary storage functionality.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph*{RAW~\cite{raw} \& VIDa~\cite{vida}}
The RAW system and its VIDa extension aim to query heterogeneous data sources transparently, without loading data into a database. RAW generates access paths just-in-time to adapt to the underlying data files and to the incoming queries. \texttt{SCANRAW} integrates external I/O libraries to access different data formats, e.g., BAM and FITS. Furthermore, \texttt{SCANRAW} measures the performance of the library dynamically in order to decide whether to load the data into database to improve the execution of subsequent queries.

\paragraph*{Impala~\cite{impala}}
Impala is an open source massively parallel processing SQL query engine for data stored in a computer cluster running Hadoop\footnote{\url{http://hadoop.apache.org}}. Impala brings scalable parallel database technology to Hadoop, enabling users to issue low-latency SQL queries to data stored in HDFS and HBase\footnote{\url{http://hbase.apache.org/}} without requiring data movement or transformation. Impala applies task-parallelism to convert raw data into binary format for execution. When Impala executes a query from a raw file, it has to first retrieve the data from HDFS, the underlying file system. Therefore, the execution time for the first query cannot be fully controlled by Impala. Compared to Impala, \texttt{SCANRAW} applies super-scalar pipeline parallelism in order to maximize the hardware throughput.

